Bivariate Hierarchical Bayesian Model for Combining Summary Measures and their Uncertainties from Multiple Sources

It is often of interest to combine available estimates of a similar quantity from multiple data sources. When the corresponding variances of each estimate are also available, a model should take into account the uncertainty of the estimates themselves as well as the uncertainty in the estimation of variances. In addition, if there exists a strong association between estimates and their variances, the correlation between these two quantities should also be considered. In this paper, we propose a bivariate hierarchical Bayesian model that jointly models the estimates and their estimated variances assuming a correlation between these two measures. We conduct simulations to explore the performance of the proposed bivariate Bayesian model and compare it to other commonly used methods under different correlation scenarios. The proposed bivariate Bayesian model has a wide range of applications. We illustrate its application in three very different areas: PET brain imaging studies, meta-analysis, and small area estimation.

==> figtex/fig13-muadds.tex <==
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=5.5in]{figs/sim-mu_t_bw.pdf}
\end{center}
\caption{Comparison of BBM and UBM to the three non-Bayesian methods for estimating the population overall mean with $\rho_1$ and $\rho_2$ values taking different values when the variation between summary measures from different sources is small, where mean vector is $(\mu_\theta = 10, \mu_\sigma =0.2)^T$ and variance components are $r_\theta =3, r_\sigma=0.1$, and $\sigma_{s_i} = 1$. The violin plot presents the distribution of estimates and the number above shows the 95\% CI coverage rate based on $500$ simulations.}
\label{f-13}
\end{figure}

==> tabtex/tab1-mu.tex <==


\begin{table}[!ht]
\caption{Comparison of estimation for the population mean using five different methods under different correlations.}
\label{t-1}
\begin{center} 
\scalebox{0.75}{
\begin{tabular}{c|c|ccc|ccc|ccc}
\hline
\textbf{Correlation} & &
\multicolumn{3}{c}{\textbf{$\rho=0.3$}} & \multicolumn{3}{c}{\textbf{$\rho=0.5$}} &  \multicolumn{3}{c}{\textbf{$\rho=0.7$}} \\\hline
Scenario    & $\mu=10$    & Bias   & MSE  & Coverage & Bias   & MSE   & Coverage & Bias  & MSE   & Coverage \\\hline
$\rho_1=0, \rho_2 = 0$   & Raw   & 0.05  & 7.74 & 0.93 & 0.05  & 7.74 & 0.93 & 0.05  & 7.74 & 0.93 \\
            & Weighted &0.03  & 4.62 & 0.89 & 0.03  & 4.62 & 0.89 & 0.03  & 4.62 & 0.89     \\
            & Trimmed &-0.01 & 2.41 & 0.94 & -0.01 & 2.41 & 0.94 & -0.01 & 2.41 & 0.94     \\
            & UBM   & -0.02 & 2.54 & 0.95 & -0.02 & 2.54 & 0.95 & -0.02 & 2.54 & 0.95     \\
            & BBM   & -0.04 & 1.51 & 0.96 & -0.04 & 1.51 & 0.96 & -0.04 & 1.51 & 0.96     \\\hline
$\rho_1 =\rho, \rho_2 = 0$    & Raw   & 0.05  & 7.74 & 0.93 & 0.05  & 7.72 & 0.93 & 0.05  & 7.74 & 0.93   \\
            & Weighted &  -1.39 & 7.1  & 0.79 & -2.29 & 11.3 & 0.61 & -3.16 & 17.8 & 0.43    \\
            & Trimmed     & -1.51 & 4.81 & 0.8  & -2.5  & 9.21 & 0.57 & -3.47 & 15.8 & 0.37     \\
            & UBM            & -1.5  & 4.77 & 0.84 & -2.46 & 8.62 & 0.64 & -3.41 & 14.3 & 0.39     \\
            & BBM             & 0.14  & 1.5  & 0.95 & 0.31  & 1.61 & 0.94 & 0.57  & 1.78 & 0.93    \\\hline
$\rho_1 =  0, \rho_2=\rho$    & Raw    & 0.08  & 8.53 & 0.94 & 0.07  & 9.55 & 0.94 & 0.04  & 10.6 & 0.94     \\
            & Weighted & -1.21 & 6.38 & 0.82 & -2.12 & 9.81 & 0.69 & -2.91 & 14.1 & 0.54   \\
            & Trimmed     & -1.01 & 3.58 & 0.85 & -1.68 & 5.57 & 0.74 & -2.3  & 8.26 & 0.6     \\
            & UBM            & -0.44 & 2.73 & 0.92 & -0.73 & 3.09 & 0.87 & -1.04 & 3.59 & 0.83     \\
            & BBM             & -0.56 & 1.83 & 0.93 & -0.88 & 2.33 & 0.89 & -1.23 & 3.07 & 0.83  \\\hline
$\rho_1=\rho, \rho_2 =\rho$ & Raw    & 0.08  & 8.52 & 0.94 & 0.07  & 9.56 & 0.93 & 0.04  & 10.6 & 0.94  \\
            & Weighted &  -2.67 & 11.6 & 0.51 & -4.44 & 24   & 0.15 & -6    & 40.2 & 0.01     \\
            & Trimmed     & -2.55 & 8.89 & 0.54 & -4.17 & 20.1 & 0.12 & -5.72 & 35.5 & 0.01    \\
            & UBM            & -1.94 & 6.03 & 0.7  & -3.27 & 12.8 & 0.34 & -4.59 & 22.9 & 0.06     \\
            & BBM             & -0.35 & 1.62 & 0.94 & -0.49 & 1.78 & 0.92 & -0.62 & 1.87 & 0.9 \\\hline
\end{tabular}}
\end{center}
\end{table}

==> tabtex/tab3-beta02.tex <==



\begin{scriptsize}
\LTcapwidth=\textwidth
\begin{longtable}{c|c|ccc|ccc|ccc}
\caption{Comparison of estimation for the regression coefficients of intercept and categorical variable using five methods under different correlations.}
\label{t-3}\\
\hline
\textbf{Correlation} & &
\multicolumn{3}{c}{\textbf{$\rho=0.3$}} & \multicolumn{3}{c}{\textbf{$\rho=0.5$}} &  \multicolumn{3}{c}{\textbf{$\rho=0.7$}} \\\hline
Scenario    & $\beta_{\theta,0}=5$   & Bias & MSE   & Coverage & Bias  & MSE   & Coverage & Bias  & MSE   & Coverage \\\hline
\endfirsthead
\hline
\textbf{Correlation} & &
\multicolumn{3}{c}{\textbf{$\rho=0.3$}} & \multicolumn{3}{c}{\textbf{$\rho=0.5$}} &  \multicolumn{3}{c}{\textbf{$\rho=0.7$}} \\\hline
Scenario    & $\beta_{\theta,0}=5$   & Bias & MSE   & Coverage & Bias  & MSE   & Coverage & Bias  & MSE   & Coverage \\\hline
\endhead
\hline
\endfoot
$\rho_1=0$,$\rho_2 = 0$ & LR          & -0.04 & 8.27  & 0.97 & -0.04 & 8.27  & 0.97 & -0.04 & 8.27  & 0.97 \\
         & WLR         & -0.13 & 7.57  & 0.48 & -0.13 & 7.57  & 0.48 & -0.13 & 7.57  & 0.48 \\
         & TWLR        & -0.05 & 4.22  & 0.55 & -0.05 & 4.22  & 0.55 & -0.05 & 4.22  & 0.55 \\
         & UBM         & -0.04 & 1.5   & 0.91 & -0.04 & 1.5   & 0.91 & -0.04 & 1.5   & 0.91 \\
         & BBM         & -0.06 & 1.03  & 0.93 & -0.06 & 1.03  & 0.93 & -0.06 & 1.03  & 0.93 \\\hline
$\rho_1 =\rho, \rho_2 = 0$  & LR          & -0.04 & 8.26  & 0.97 & -0.04 & 7.78  & 0.97 & 0     & 6.55  & 0.97 \\
         & WLR         & -0.72 & 7.66  & 0.47 & -1.12 & 8.41  & 0.44 & -1.44 & 9.27  & 0.42 \\
         & TWLR        & -0.68 & 4.63  & 0.56 & -1.12 & 5.53  & 0.54 & -1.49 & 6.5   & 0.46 \\
         & UBM         & -0.92 & 2.42  & 0.84 & -1.5  & 3.94  & 0.74 & -2.03 & 5.82  & 0.56 \\
         & BBM         & 0.06  & 0.99  & 0.93 & 0.16  & 0.96  & 0.95 & 0.2   & 0.91  & 0.94 \\\hline
$\rho_1 =  0, \rho_2 =\rho$  & LR          & 0.06  & 8.14  & 0.96 & -0.01 & 8.28  & 0.97 & 0.07  & 7.78  & 0.97 \\
         & WLR         & -1.14 & 9.15  & 0.41 & -1.86 & 11.17 & 0.36 & -2.74 & 14.01 & 0.26 \\
         & TWLR        &  -0.96 & 5.27  & 0.49 & -1.68 & 7.15  & 0.4  & -2.43 & 9.64  & 0.26 \\
         & UBM         & -0.39 & 1.71  & 0.87 & -0.6  & 1.9   & 0.82 & -0.82 & 2.26  & 0.74 \\
         & BBM         & -0.2  & 1.03  & 0.93 & -0.32 & 1.08  & 0.93 & -0.46 & 1.12  & 0.91   \\\hline
$\rho_1 =\rho, \rho_2 =\rho$  & LR      &  -0.03 & 7.72  & 0.96 & 0.06  & 8.34  & 0.97 & 0.07  & 7.73  & 0.97 \\
         & WLR         & -1.74 & 10.74 & 0.35 & -2.93 & 15.23 & 0.18 & -4.1  & 22.01 & 0.1  \\
         & TWLR        & -1.63 & 6.42  & 0.41 & -2.79 & 11.09 & 0.17 & -3.94 & 18.57 & 0.06 \\
         & UBM         & -1.29 & 3.08  & 0.71 & -2.1  & 5.87  & 0.44 & -2.91 & 10.13 & 0.13 \\
         & BBM         & -0.09 & 0.97  & 0.95 & -0.11 & 0.92  & 0.95 & -0.15 & 0.87  & 0.95 \\\hline

            & $\beta_{\theta,2}=1$          & Bias & MSE   & Coverage & Bias & MSE   & Coverage & Bias  & MSE   & Coverage \\\hline
$\rho_1=0, \rho_2 = 0$ & LR          & 0.09  & 35.74 & 0.95 & 0.09  & 35.74 & 0.95 & 0.09  & 35.74 & 0.95 \\
         & WLR         & 0.22  & 10.54 & 0.6  & 0.22  & 10.54 & 0.6  & 0.22  & 10.54 & 0.6  \\
         & TWLR        & 0.14  & 7.9   & 0.64 & 0.14  & 7.9   & 0.64 & 0.14  & 7.9   & 0.64 \\
         & UBM         & 0.03  & 5.31  & 0.92 & 0.03  & 5.31  & 0.92 & 0.03  & 5.31  & 0.92 \\
         & BBM         & 0.06  & 3.34  & 0.94 & 0.06  & 3.34  & 0.94 & 0.06  & 3.34  & 0.94 \\\hline
$\rho_1 =\rho, \rho_2 = 0$  & LR          &0.09  & 35.7  & 0.95 & 0.1   & 35.84 & 0.96 & 0.18  & 46.11 & 0.95 \\
         & WLR         & 0.28  & 10.95 & 0.61 & 0.28  & 11.57 & 0.63 & 0.27  & 11.33 & 0.64 \\
         & TWLR        & 0.23  & 8.47  & 0.64 & 0.25  & 9.02  & 0.65 & 0.26  & 8.8   & 0.67 \\
         & UBM         & 0.29  & 5.58  & 0.92 & 0.42  & 5.79  & 0.94 & 0.53  & 7.02  & 0.93 \\
         & BBM         & 0.06  & 3.23  & 0.94 & 0.01  & 3.08  & 0.94 & 0.05  & 3.06  & 0.95 \\\hline
$\rho_1 =  0, \rho_2 =\rho$  & LR          &  -0.02 & 29.72 & 0.96 & -0.06 & 30.46 & 0.95 & -0.1  & 27.69 & 0.96 \\
         & WLR         & 0.3   & 11.23 & 0.63 & 0.52  & 11.07 & 0.65 & 0.87  & 10.24 & 0.65 \\
         & TWLR        & 0.13  & 7.47  & 0.67 & 0.34  & 7.98  & 0.67 & 0.58  & 7.89  & 0.7  \\
         & UBM         & 0.02  & 4.94  & 0.92 & 0     & 4.92  & 0.92 & 0.06  & 4.53  & 0.94 \\
         & BBM         &0.06  & 3.32  & 0.94 & 0.09  & 3.28  & 0.93 & 0.12  & 2.94  & 0.93 \\\hline
$\rho_1 =\rho, \rho_2 =\rho$    & LR          &-0.06 & 29.56 & 0.96 & -0.07 & 27.29 & 0.96 & 0.07  & 23.69 & 0.95 \\
         & WLR         & 0.36  & 11.43 & 0.63 & 0.72  & 9.88  & 0.66 & 0.9   & 8.24  & 0.65 \\
         & TWLR        & 0.22  & 7.05  & 0.66 & 0.56  & 6.51  & 0.69 & 0.73  & 6.11  & 0.71 \\
         & UBM         & 0.33  & 4.8   & 0.94 & 0.59  & 4.58  & 0.95 & 0.67  & 6.36  & 0.95 \\
         & BBM         &  0.06  & 3.19  & 0.94 & 0.12  & 2.93  & 0.94 & 0.15  & 2.64  & 0.94 \\\hline
\end{longtable}
\end{scriptsize}

==> tabtex/tab4-pet.tex <==



\begin{table}[!h]
\caption{Estimation of average binding potential of \texttt{amygdala} region without and with adjusting for covariates.}
\label{t-4}
\begin{center}
\scalebox{0.85}{
\begin{tabular}{r|c|c|c|c}
\hline
\textbf{Method} &\textbf{Without covariates} &\multicolumn{3}{c}{\textbf{With covariates}} \\\hline
& $\hat{\mu}$(95\%CI)  & $\hat{\beta}_{diag}$(95\%CI)   & $\hat{\beta}_{age}$(95\%CI)  & $\hat{\beta}_{gender}$(95\%CI) \\\hline
Raw/LR           & 111.58(103.68,119.47) & -9.51(-26.69,7.67)    & -0.24(-0.97,0.49) & -8.86(-24.67,6.94) \\
Weighted/WLR     & 74.91(55.09,101.8)    & -41.99(-61.52,-22.47) & 0.42(-0.33,1.18)  & 21.71(4.93,38.5)   \\
Trimmed/TWLR & 91.38(76.72,103.51)   & -23.08(-39.35,-6.8)   & 0.04(-0.6,0.67)   & 2.78(-11.6,17.17)  \\
UBM           & 100.97(93.11,109.31)  & -15.91(-33.82,2.38)   & -0.16(-0.94,0.57) & -1.96(-17.9,13.4)  \\
BBM           & 112.2(105.25,119.61)  & -8.85(-24.47,5.6)     & -0.16(-0.87,0.5)  & -8.48(-22.78,5.37)\\\hline    
\end{tabular}}
\end{center}
\end{table}





==> tabtex/tab5-fars.tex <==



\begin{footnotesize}
\LTcapwidth=\textwidth
\begin{longtable}{r|p{1.2in}p{1.2in}p{1.2in}}
\kill
\caption{Comparison of the estimates and confident/credible intervals of state-level average number of vehicles involved in a crash using FARS 2017 data.}
\label{t-5}\\
\hline
\textbf{State} & \textbf{raw mean $y_i$} & \textbf{UBM $\hat{\theta}_i$}  & \textbf{BBM $\Tilde{\theta}_i$}\\\hline
\endfirsthead
\hline
\textbf{Region} & \textbf{raw mean $y_i$} & \textbf{UBM  $\hat{\theta}_i$}  & \textbf{BBM $\Tilde{\theta}_i$} \\\hline
\endhead
\hline
\endfoot
Alabama              & 1.49(1.44,1.54) & 1.51(1.47,1.55) & 1.51(1.46,1.55) \\
Alaska               & 1.37(1.24,1.5)  & 1.48(1.41,1.55) & 1.48(1.4,1.56)  \\
Arizona              & 1.56(1.5,1.62)  & 1.55(1.5,1.59)  & 1.55(1.49,1.61) \\
Arkansas             & 1.52(1.46,1.58) & 1.53(1.48,1.58) & 1.54(1.48,1.6)  \\
California           & 1.61(1.58,1.64) & 1.62(1.59,1.64) & 1.61(1.59,1.63) \\
Colorado             & 1.61(1.54,1.68) & 1.57(1.52,1.63) & 1.56(1.48,1.63) \\
Connecticut          & 1.54(1.46,1.62) & 1.55(1.49,1.6)  & 1.55(1.49,1.6)  \\
Delaware             & 1.59(1.46,1.72) & 1.55(1.49,1.62) & 1.56(1.5,1.62)  \\
District of Columbia & 1.48(1.21,1.75) & 1.53(1.45,1.61) & 1.51(1.44,1.59) \\
Florida              & 1.62(1.59,1.65) & 1.62(1.59,1.65) & 1.62(1.59,1.65) \\
Georgia              & 1.62(1.57,1.67) & 1.61(1.57,1.65) & 1.6(1.56,1.64)  \\
Hawaii               & 1.56(1.42,1.7)  & 1.52(1.46,1.6)  & 1.53(1.46,1.6)  \\
Idaho                & 1.5(1.41,1.59)  & 1.49(1.43,1.55) & 1.5(1.43,1.55)  \\
Illinois             & 1.62(1.57,1.67) & 1.6(1.56,1.65)  & 1.61(1.57,1.64) \\
Indiana              & 1.6(1.55,1.65)  & 1.59(1.55,1.63) & 1.59(1.54,1.64) \\
Iowa                 & 1.53(1.46,1.6)  & 1.54(1.49,1.6)  & 1.54(1.49,1.59) \\
Kansas               & 1.55(1.48,1.62) & 1.53(1.48,1.58) & 1.54(1.49,1.58) \\
Kentucky             & 1.55(1.5,1.6)   & 1.54(1.5,1.58)  & 1.54(1.49,1.58) \\
Louisiana            & 1.54(1.48,1.6)  & 1.54(1.5,1.59)  & 1.55(1.5,1.6)   \\
Maine                & 1.6(1.48,1.72)  & 1.55(1.49,1.62) & 1.55(1.48,1.62) \\
Maryland             & 1.64(1.56,1.72) & 1.59(1.53,1.65) & 1.6(1.54,1.65)  \\
Massachusetts        & 1.45(1.38,1.52) & 1.51(1.44,1.56) & 1.51(1.44,1.58) \\
Michigan             & 1.63(1.58,1.68) & 1.61(1.57,1.66) & 1.61(1.55,1.65) \\
Minnesota            & 1.59(1.51,1.67) & 1.57(1.52,1.62) & 1.58(1.53,1.62) \\
Mississippi          & 1.54(1.48,1.6)  & 1.53(1.48,1.57) & 1.53(1.48,1.58) \\
Missouri             & 1.56(1.51,1.61) & 1.56(1.52,1.6)  & 1.57(1.52,1.61) \\
Montana              & 1.39(1.31,1.47) & 1.47(1.4,1.53)  & 1.49(1.4,1.57)  \\
Nebraska             & 1.56(1.46,1.66) & 1.53(1.47,1.59) & 1.54(1.49,1.59) \\
Nevada               & 1.6(1.48,1.72)  & 1.54(1.47,1.62) & 1.54(1.46,1.61) \\
New Hampshire        & 1.5(1.37,1.63)  & 1.53(1.46,1.59) & 1.53(1.47,1.59) \\
New Jersey           & 1.56(1.49,1.63) & 1.56(1.5,1.61)  & 1.56(1.51,1.61) \\
New Mexico           & 1.6(1.43,1.77)  & 1.53(1.46,1.6)  & 1.54(1.47,1.62) \\
New York             & 1.56(1.51,1.61) & 1.56(1.51,1.61) & 1.56(1.48,1.64) \\
North Carolina       & 1.56(1.52,1.6)  & 1.56(1.52,1.59) & 1.56(1.52,1.59) \\
North Dakota         & 1.45(1.34,1.56) & 1.51(1.44,1.58) & 1.51(1.44,1.58) \\
Ohio                 & 1.58(1.54,1.62) & 1.58(1.55,1.62) & 1.58(1.55,1.62) \\
Oklahoma             & 1.54(1.48,1.6)  & 1.55(1.5,1.59)  & 1.55(1.5,1.6)   \\
Oregon               & 1.5(1.42,1.58)  & 1.52(1.46,1.57) & 1.52(1.45,1.58) \\
Pennsylvania         & 1.65(1.57,1.73) & 1.61(1.56,1.67) & 1.63(1.59,1.67) \\
Rhode Island         & 1.46(1.29,1.63) & 1.53(1.46,1.58) & 1.51(1.45,1.58) \\
South Carolina       & 1.5(1.46,1.54)  & 1.51(1.47,1.55) & 1.51(1.46,1.55) \\
South Dakota         & 1.43(1.33,1.53) & 1.49(1.41,1.54) & 1.47(1.41,1.53) \\
Tennessee            & 1.55(1.5,1.6)   & 1.54(1.5,1.59)  & 1.54(1.51,1.58) \\
Texas                & 1.61(1.58,1.64) & 1.62(1.59,1.64) & 1.61(1.6,1.64)  \\
Utah                 & 1.63(1.52,1.74) & 1.55(1.49,1.62) & 1.55(1.46,1.63) \\
Vermont              & 1.51(1.35,1.67) & 1.53(1.46,1.61) & 1.52(1.45,1.59) \\
Virginia             & 1.53(1.48,1.58) & 1.55(1.51,1.59) & 1.55(1.5,1.59)  \\
Washington           & 1.59(1.52,1.66) & 1.56(1.51,1.62) & 1.56(1.5,1.62)  \\
West Virginia        & 1.43(1.35,1.51) & 1.49(1.43,1.55) & 1.5(1.43,1.57)  \\
Wisconsin            & 1.53(1.48,1.58) & 1.53(1.49,1.57) & 1.53(1.5,1.57)  \\
Wyoming              & 1.39(1.28,1.5)  & 1.46(1.38,1.52) & 1.45(1.38,1.53) \\\hline
\end{longtable}
\end{footnotesize}


==> tabtex/tab6-comp.tex <==

\begin{table}
    \caption{CPU seconds and maximum memory required for 10 replications for UBM and BBM with $n=50$ simulation sample and parameters $\mu=10, \rho_1 = 0, \rho_2 = 0.3$. }
    \label{t-6}
    \begin{center}
    \scalebox{1.0}{
    \begin{tabular}{r|c|c}
    \hline
    \textbf{Method} &\textbf{CPU time} &{\textbf{Max. memory/given memory}} \\\hline
    UBM     & 124 s & 2.098G /8G \\
    BBM     & 80764 s   & 2.214G /8G \\
    BBM with fixed $\sigma_{s_i}$  & 10060 s    & 3.606G /8G \\\hline    
    \end{tabular}}
    \end{center}
\end{table}

==> tabtex/tab7-meta.tex <==

\begin{table}
    \caption{Comparison of combined estimates and and 95\% CIs for population-level log odds ratio of risk of respiratory tract infection by comparing the treatment group to placebo}
    \label{t-7}
    \begin{center}
    \begin{tabular}{r|c|c|c|c}
    \hline
    \textbf{Method} &\textbf{Log OR} &\textbf{95\% CI} & \textbf{\makecell{Between trial\\ variance($\tau^2$ or $r_\theta^2$)}} & \textbf{95\% CI} \\\hline
    Raw      & -1.64  & (-2.08, -1.19)  & 0 & -\\
    Weighted & -0.947 & (-1.36, -0.692) & 0 & - \\
    Trimmed  & -0.947 & (-1.39, -0.692) & 0 & -   \\
    UBM      & -1.32  & (-1.77, -0.930) & 0.735 & (0.377,1.21)    \\
    BBM      & -1.66  & (-2.13, -1.22) & 0.879 & (0.365,1.34)   \\\hline    
    \end{tabular}
    \end{center}
\end{table}
